Hyper-Kamiokande Physics Opportunities

We propose the Hyper-Kamiokande (Hyper-K) detector as a next generation un- derground water Cherenkov detector. It will serve as a far detector of a long base- line neutrino oscillation experiment envisioned for the upgraded J-PARC beam, and as a detector capable of observing, far beyond the sensitivity of the Super-Kamiokande (Super-K) detector, proton decays, atmospheric neutrinos, and neutrinos from astro- physical origins. The current baseline design of Hyper-K is based on the highly suc- cessful Super-K detector, taking full advantage of a well-proven technology. Hyper-K consists of two cylindrical tanks lying side-by-side, the outer dimensions of each tank being 48(W) x54(H) x 250(L) m3. The total (fiducial) mass of the detector is 0.99 (0.56) million metric tons, which is about 20 (25) times larger than that of Super-K. This set of three one- page whitepapers prepared for the US Snowmass process describes the opportunities for future physics discoveries at the Hyper-K facility with beam, atmospheric and astrophysical neutrinos.

==> author-full.tex <==
\begin{center}
\vspace{0.0in} \textbf{\Large The Hyper-Kamiokande Working Group} \vspace{.15in}
\end{center}

\noindent
{\bf Boston University (USA):}
E. Kearns,  J.L. Stone \authorspace

\noindent
{\bf Brookhaven National Laboratory (USA):}
D.E. Jaffe,  J. Ling,  B. Viren,  M. Yeh \authorspace

\noindent
{\bf Duke University (USA):}
T. Akiri, A. Himmel,  K. Scholberg, C.W. Walter \authorspace

\noindent 
{\bf Earthquake Research Institute, The University of Tokyo (Japan):}
 A. Taketa,  H.K.M. Tanaka \authorspace

\noindent
{\bf ETH Zurich (Switzerland):}
A. Rubbia \authorspace

\noindent
{\bf Institute for Nuclear Research (Russia):}
A. Izmaylov, M. Khabibullin,  Yu. Kudenko  \authorspace

\noindent
{\bf Imperial College London (UK):}
Y. Uchida, M.O. Wascko \authorspace

\noindent 
{\bf Kamioka Observatory, ICRR, The University of Tokyo (Japan):}
K. Abe, Y. Haga, Y. Hayato, J. Kameda, Y. Kishimoto, Y. Koshio,
L. Marti, M. Miura, S. Moriyama, M. Nakahata, S. Nakayama, H. Sekiya,
M. Shiozawa, Y. Suzuki, A. Takeda, H. Tanaka, T. Tomura, R. Wendell
\authorspace

\noindent
{\bf KEK (Japan):}
K.Nakamura \authorspace

\noindent
{\bf Kobe University (Japan) :}
 A. T. Suzuki, Y. Takeuchi \authorspace

\noindent
{\bf Kyoto University (Japan):}
S. Hirota, K. Huang, A. K. Ichikawa, M. Ikeda, A. Minamino, T. Nakaya,
K. Tateishi \authorspace

\noindent
{\bf Lancaster University (UK):}
L.L. Kormos, P.N. Ratoff \authorspace

\noindent
{\bf Los Alamos National Laboratory (USA):}
C. Mauger, G. Sinnis \authorspace

\noindent 
{\bf Louisiana State University (USA):}
F.d.M. Blaszczyk,  J. Insler, T. Kutter, O. Perevozchikov, M. Tzanov \authorspace

\noindent
{\bf Miyagi University of Education (Japan):}
Y.Fukuda \authorspace

\noindent
{\bf Nagoya University (Japan):}
K.Choi, T. Iijima,  Y. Itow \authorspace

\noindent
{\bf  The Ohio State University (USA):}
C. Rott \authorspace

\noindent
{\bf Okayama University (Japan):}
H. Ishino, T. Mori, M. Sakuda, T. Yano \authorspace

\noindent
{\bf Osaka City University (Japan):}
Y. Seiya,  K. Yamamoto \authorspace

\noindent 
{\bf Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (Brazil):}
H. Minakata, H. Nunokawa \authorspace

\noindent
{\bf Queen Mary, University of London (UK):}
F. Di Lodovico, J.R. Wilson \authorspace

\noindent
{\bf STFC Rutherford Appleton Laboratory (UK):}
D. Wark \authorspace

\noindent
{\bf Tohoku University (Japan):}
K. Inoue,  M. Koga, I. Shimizu \authorspace

\noindent
{\bf Research Center for Cosmic Neutrinos, ICRR, The University of Tokyo (Japan):}
T. Irvine, T. Kajita, I. Kametani, Y. Nishimura, K. Okumura, E. Richard \authorspace

\noindent
{\bf Tokyo Institute of Technology (Japan):}
M. Ishitsuka, M. Kuze, Y. Okajima \authorspace

\noindent
{\bf TRIUMF (Canada):}
P. Gumplinger, A. Konaka, T. Lindner, K. Mahn, J.-M. Poutissou, F.
Retiere, M.J. Wilking \authorspace

\noindent
{\bf University of British Columbia (Canada):}
S.M. Oser, H.A. Tanaka \authorspace

\noindent
{\bf University of Geneva (Switzerland):}
Alain Blondel, Alessandro Bravar, Fanny Dufour, Yordan Karadhzov, Alex
Korzenev, Etam Noah, Melody Ravonel, Mark Rayner, Ruslan Asfandiyarov,
Alexis Haesler, Carlos Martin, Enrico Scantamburlo \authorspace

\noindent
{\bf The University of Tokyo (Japan):}
H. Aihara, Y. Suda, M. Yokoyama \authorspace

\noindent
{\bf University of Toronto (Canada):}
J.F. Martin \authorspace

\noindent
{\bf University of California, Davis (USA):}
R.Svoboda, M.Bergevin \\

\noindent
{\bf University of California, Irvine (USA):}
G. Carminati, S. Horiuchi, W.R. Kropp, S. Mine, M.B. Smy, H.W. Sobel, M.R. Vagins \authorspace

\noindent
{\bf University of Liverpool (UK):}
N. McCauley \authorspace

\noindent
{\bf University of Sheffield (UK):}
J.D. Perkin, L.F. Thompson \authorspace

\noindent
{\bf University of Washington (USA):}
J. Detwiler, N. Tolich, R. J. Wilkes \authorspace

\noindent
{\bf University of Warwick (UK):}
G.J. Barker, S. Boyd, D.R. Hadley, M.D. Haigh \authorspace

\noindent
{\bf University of Winnipeg (Canada):}
B. Jamieson \authorspace

\noindent
{\bf Virginia Tech (USA):}
S. M. Manecki, C. Mariani, S. D. Rountree, R. B. Vogelaar \authorspace

\noindent
{\bf York University (Canada):}
S. Bhadra, M. Hartz \authorspace


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "hk-whitepaper.tex"
%%% End: 


==> pdk.tex <==
\noindent
{\bf \large Exploring the Ultimate Unification of Forces \\
by Studying Nucleon Decay}

{\vskip 0.1in}

\noindent
Overview of proton decay in Hyper-K.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "hk-whitepaper.tex"
%%% End: 

